CLIMB: Data Foundations for Large Scale Multimodal Clinical Foundation Models

Recent advances in clinical AI have enabled remarkable progress across many clinical domains. However, existing benchmarks and models are primarily limited to a small set of modalities and tasks, which hinders the development of large-scale multimodal methods that can make holistic assessments of patient health and well-being. To bridge this gap, we introduce Clinical Large-Scale Integrative Multimodal Benchmark (CLIMB), a comprehensive clinical benchmark unifying diverse clinical data across imaging, language, temporal, and graph modalities. CLIMB comprises 4.51 million patient samples totaling 19.01 terabytes distributed across 2D imaging, 3D video, time series, graphs, and multimodal data. Through extensive empirical evaluation, we demonstrate that multitask pretraining significantly improves performance on understudied domains, achieving up to 29% improvement in ultrasound and 23% in ECG analysis over single-task learning. Pretraining on CLIMB also effectively improves models' generalization capability to new tasks, and strong unimodal encoder performance translates well to multimodal performance when paired with task-appropriate fusion strategies. Our findings provide a foundation for new architecture designs and pretraining strategies to advance clinical AI research. Code is released at https://github.com/DDVD233/climb.

==> algorithms/download.tex <==
\begin{algorithm*}
\caption{Dataset loading and model training with High-Modality framework}
\label{alg:framework}
\begin{lstlisting}[language=Python]
from transformers import Trainer
from high_modality.datasets import *
from high_modality.models import ConvNextV2Classifier

# List of datasets to load, could be all datasets (AllDatasets),
# modality-specific (XRAY, MRI) or individual datasets (CBIS, MIMIC_IV)
datasets = [XRAY, CBIS, PATHOLOGY]
train_dataset, val_dataset, test_dataset = load_datasets(datasets, 
    download=True, base_dir='/path/to/datasets')
train_loader, val_loader, test_loader = init_dataloader(train_dataset, val_dataset, test_dataset, batch_size=32)

model = ConvNextV2Classifier()

# Train with huggingface trainer
trainer = Trainer(model=model, train_dataset=train_loader, eval_dataset=val_loader)
trainer.train()
trainer.evaluate()
\end{lstlisting}
\end{algorithm*}
% \vspace{-3em}

==> algorithms/framework.tex <==
\begin{algorithm}[t]
\caption{Loading and training with \datasetname~framework}
\label{alg:framework}
\tiny
\begin{lstlisting}[language=Python]
from transformers import Trainer
from high_modality.datasets import *
from high_modality.models import ConvNextV2Classifier

datasets = [XRAY, CBIS, PATHOLOGY]
train_dataset, val_dataset, test_dataset = load_datasets(datasets, download=True, base_dir='/path/to/datasets')

model = ConvNextV2Classifier()
trainer = Trainer(model=model, train_dataset=train_dataset, eval_dataset=val_dataset)
trainer.train()
trainer.evaluate()
\end{lstlisting}
\vspace{-1em}
\end{algorithm}

% # List of datasets to load, could be all datasets (AllDatasets),
% # modality-specific (XRAY, MRI) or individual datasets (CBIS, MIMIC_IV)
% # Train with huggingface trainer

==> tables/llm_by_modality.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Performance comparison of zero-shot and fine-tuned LLaVa-Med.} LLaVa-Med is the current SoTA LVLM model for clinical QA tasks. Both \datasetname-ConvNextv2 and LLaVa-Med are trained and evaluated on \datasetname~in a comparable, close-ended manner. While directly fine-tuning the LLM on \datasetname-QA improves performance over zero-shot cases, they still lag behind SoTA multitask encoders, namely \datasetname-ConvNextv2, the SoTA multitask encoder trained on \datasetname.}
\vspace{1mm}

\label{tab:llava_zero_vs_finetune}
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Zero-Shot}} & \multicolumn{3}{c|}{\textbf{Fine-Tuned}} & \multicolumn{3}{c}{\textbf{Qwen ZS}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{Acc} & \textbf{Sens} & \textbf{Spe} & \textbf{Acc} & \textbf{Sens} & \textbf{Spe} & \textbf{Acc} & \textbf{Sens} & \textbf{Spe} \\
\midrule
Chest X-ray   & .088 & .192 & .808 & .309 & .207 & .795 & .881 & .143 & .952 \\
MRI            & .363 & .473 & .650 & .480 & .375 & .625 & .923 & .353 & .957 \\
Ultrasound     & .448 & .427 & .640 & .579 & .389 & .611 & .395 & .218 & .506 \\
Mammography    & .049 & .203 & .800 & .741 & .300 & .700 & .942 & .117 & .970 \\
Dermoscopy     & .466 & .296 & .700 & .673 & .245 & .756 & .949 & .230 & .973 \\
Fundus         & .434 & .202 & .794 & .578 & .217 & .783 & .942 & .426 & .969 \\
CT             & .448 & .424 & .575 & .788 & .435 & .585 & .978 & .302 & .989 \\
Endoscopic     & .000 & 1.00 & .000 & .296 & .143 & .857 & - & - & - \\
\midrule
Average & .287 & .402 & .621 & .555 & .289 & .714 & - & - & - \\
\rowcolor{gray!20} \textbf{\datasetname-ConvNextv2} & - & - & - & \textbf{.877} & \textbf{.806} & \textbf{.787} & - & - & - \\
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

==> tables/tables_of_figures/one_shot_table.tex <==
\begin{table*}[htbp]
\centering
\caption{\textbf{Performance comparison of different pretraining strategies across medical imaging modalities.} Performance is measured in AUC (Area under the receiver operating characteristic curve) for each modality.}
\label{tab:pretrain_comparison}
\resizebox{\textwidth}{!}{
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccccccc}
\toprule
\textbf{Pretrain Dataset} & \textbf{Chest X-Ray} & \textbf{Dermoscopy} & \textbf{CT Scan} & \textbf{Fundus} & \textbf{Pathology} & \textbf{Mammography} & \textbf{Ultrasound} & \textbf{ECG} \\
\midrule
PT on Ours & .794 & .760 & .664 & .705 & .554 & .645 & .614 & .545 \\
PT on Standard Datasets & .779 & .624 & .516 & .634 & .540 & .593 & .422 & .495 \\
\bottomrule
\end{tabular}
}
\end{table*}
